Differentially Private Stochastic Coordinate Descent

In this paper we tackle the challenge of making the stochastic coordinate descent algorithm differentially private. Compared to the classical gradient descent algorithm where updates operate on a single model vector and controlled noise addition to this vector suffices to hide critical information about individuals, stochastic coordinate descent crucially relies on keeping auxiliary information in memory during training. This auxiliary information provides an additional privacy leak and poses the major challenge addressed in this work. Driven by the insight that under independent noise addition, the consistency of the auxiliary information holds in expectation, we present DP-SCD, the first differentially private stochastic coordinate descent algorithm. We analyze our new method theoretically and argue that decoupling and parallelizing coordinate updates is essential for its utility. On the empirical side we demonstrate competitive performance against the popular stochastic gradient descent alternative (DP-SGD) while requiring significantly less tuning.

==> Makefile <==
.PHONY: FORCE all clean distclean

ifndef TARGET
TARGET=main
endif
.SUFFIXES: .pdf .ps .dvi .tex

all: $(TARGET).pdf

rebuttal_ijcai.pdf: rebuttal_ijcai.tex FORCE
	latexmk -pdf -g -pdflatex="pdflatex -synctex=1" -use-make rebuttal_ijcai.tex
	pdftk rebuttal_ijcai.pdf cat 7-r1 output temp_rebuttal_ijcai.pdf
	mv temp_rebuttal_ijcai.pdf rebuttal_ijcai.pdf

%.pdf: %.tex FORCE
	latexmk -pdf -pdflatex="pdflatex -synctex=1" -use-make $(TARGET).tex

clean:
	for ext in aux log toc lof lot lol dlog bbl blg out tpt fdb_latexmk; \
	do \
		$(RM) $(TARGET).$$ext ; \
	done
	$(RM) *.aux *.bak *~

distclean: clean
	$(RM) $(TARGET).pdf
	$(RM) *.d

